A $C^*$-Algebraic Approach to Parametrized Quantum Spin Systems and Their Phases in One Spatial Dimension

This thesis investigates parametrized quantum spin systems in the thermodynamic limit from a $C^*$-algebraic point of view. Our main physical result is the construction of a phase invariant for one-dimensional quantum spin chains parametrized by a topological space $X$. This invariant is constructed using $C^*$-algebraic techniques and takes values in degree one \v{C}ech cohomology $H^1(X;\mathbb{P}\mathrm{U}(\mathscr{H}))$, where $\mathbb{P}\mathrm{U}(\mathscr{H})$ is the projective unitary group of an infinite-dimensional Hilbert space $\mathscr{H}$, endowed with the strong operator topology. Using Dixmier-Douady theory [Bry93, DD63, HJJS08] one may equivalently view this as an element of $H^3(X;\mathbb{Z})$. An exactly solvable model of a one-dimensional spin system parametrized by the 3-sphere $X = \mathbb{S}^3$ is presented and it is shown that its invariant is nontrivial [WQB+22]. We also prove several mathematical results on topological aspects of the pure state space $\mathscr{P}(\mathfrak{A})$ of a $C^*$-algebra $\mathfrak{A}$. We prove that $\mathscr{P}(\mathfrak{A})$, endowed with the weak* topology, has trivial fundamental group for every UHF algebra $\mathfrak{A}$ [BHM+23]. We review the results of [SMQ+22] that show how the outputs of the GNS representation and Kadison transitivity theorem can be understood to depend continuously on their inputs. These results are expanded upon with the construction of a distinguished \v{C}ech class in $H^1(\mathscr{P}(\mathfrak{A});\mathrm{U}(1))$ that generalizes the principal $\mathrm{U}(1)$-bundle $\mathbb{S} \mathscr{H} \rightarrow \mathbb{P} \mathscr{H}$ in a representation independent way, where $\mathbb{S} \mathscr{H}$ and $\mathbb{P} \mathscr{H}$ are the unit sphere and projective Hilbert space of $\mathscr{H}$. Finally, we prove a selection theorem in the vein of [SMQ+22] for the weak* topology on $\mathscr{P}(\mathfrak{A})$.

==> dissertation_preamble.tex <==
%% Formatting
\renewcommand{\baselinestretch}{1.1}
\RequirePackage{caption}
\RequirePackage{empheq}
\RequirePackage{enumitem}
\setlist[enumerate]{topsep=4pt, itemsep=3pt}
\setlist[enumerate,1]{label=\tn{(\alph*)}}
\RequirePackage{fancyhdr}
\RequirePackage[margin=1in]{geometry}
\RequirePackage{multicol}
\RequirePackage{subfig}
\RequirePackage[dvipsnames]{xcolor}
\RequirePackage[symbol]{footmisc}
\renewcommand{\thefootnote}{\fnsymbol{footnote}}
\RequirePackage{comment}
\newcommand{\hide}[1]{}
\RequirePackage{hyperref}
\usepackage{todonotes}
\usepackage{stmaryrd}




%Make math have correct boldness in headings
\makeatletter
\g@addto@macro\bfseries{\boldmath}
\makeatother


\pagestyle{fancy}
\fancyhf{}
\renewcommand{\sectionmark}[1]{\markboth{#1}{}}
\chead{\fancyplain{}{\textit{\nouppercase{\leftmark}}}}
\cfoot{\thepage}
\setlength{\headheight}{15pt}


%% Graphics
\RequirePackage{float}
\RequirePackage{graphicx}
\RequirePackage{tikz}
\RequirePackage[compat=1.1.0]{tikz-feynman}
\tikzfeynmanset{warn luatex=false}

% tikz specifications
\usetikzlibrary{decorations.markings}
\usetikzlibrary{arrows, angles, quotes, matrix}
\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{cd}
\tikzset{snake it/.style={decorate, decoration=snake}}

%% Mathematics and physics packages
%% Math:
\RequirePackage{bm}
\RequirePackage{amsmath}
\RequirePackage{amssymb}
\RequirePackage{amsthm}
\RequirePackage[scr=dutchcal]{mathalpha}
\RequirePackage{mathtools}
\usepackage{dsfont}
\RequirePackage{accents}
\mathtoolsset{showonlyrefs,showmanualtags}


%% Physics:
\RequirePackage{cancel}
\RequirePackage[italicdiff]{physics}
\renewcommand\ket[1]{{\left|{#1}\right\rangle}}
\RequirePackage{slashed}
\RequirePackage{tensor}


%% New Environments:



\newenvironment{Proof}{\vspace{-1em}\begin{proof}\setlength{\parskip}{0.27em}}{\end{proof}\vspace{-0.05in}}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{thmdef}[theorem]{Theorem and Definition}
\newtheorem*{lemma*}{Lemma}
\newtheorem*{theorem*}{Theorem}
\newtheorem*{corollary*}{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{problem}{Problem}
\newtheorem{exercise}{Exercise}
\newtheorem{property}{Property}
\newtheorem{prop}[theorem]{Proposition}
\newtheorem{thm}[theorem]{Theorem}
\newtheorem{lem}[theorem]{Lemma}
\newtheorem{cor}[theorem]{Corollary}


\newtheorem{apptheorem}{Theorem}[chapter]
\newtheorem{appproposition}[apptheorem]{Proposition}
\newtheorem{applemma}[apptheorem]{Lemma}
\newtheorem{appcorollary}[apptheorem]{Corollary}


%Custom Named Theorem
\newtheoremstyle{named}{}{}{\itshape}{}{\bfseries}{.}{.5em}{\thmnote{#3}}
\theoremstyle{named}
\newtheorem{namedtheorem}{Theorem}

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{defn}[theorem]{Definition}
\newtheorem{rem}[theorem]{Remark}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem*{notation}{Notation}
\newtheorem{appdefinition}[apptheorem]{Definition}

\newenvironment{solution}
	{\begin{proof}[\textnormal{\bfseries Solution.}]\setlength{\parskip}{0.27em}\renewcommand{\qedsymbol}{$\blacksquare$}}
	{\end{proof}}

%Widebar command, thanks to Hendrik Vogt on TeX StackExchange.
\makeatletter
\let\save@mathaccent\mathaccent
\newcommand*\if@single[3]{%
  \setbox0\hbox{${\mathaccent"0362{#1}}^H$}%
  \setbox2\hbox{${\mathaccent"0362{\kern0pt#1}}^H$}%
  \ifdim\ht0=\ht2 #3\else #2\fi
  }
%The bar will be moved to the right by a half of \macc@kerna, which is computed by amsmath:
\newcommand*\rel@kern[1]{\kern#1\dimexpr\macc@kerna}
%If there's a superscript following the bar, then no negative kern may follow the bar;
%an additional {} makes sure that the superscript is high enough in this case:
\newcommand*\widebar[1]{\@ifnextchar^{{\wide@bar{#1}{0}}}{\wide@bar{#1}{1}}}
%Use a separate algorithm for single symbols:
\newcommand*\wide@bar[2]{\if@single{#1}{\wide@bar@{#1}{#2}{1}}{\wide@bar@{#1}{#2}{2}}}
\newcommand*\wide@bar@[3]{%
  \begingroup
  \def\mathaccent##1##2{%
%Enable nesting of accents:
    \let\mathaccent\save@mathaccent
%If there's more than a single symbol, use the first character instead (see below):
    \if#32 \let\macc@nucleus\first@char \fi
%Determine the italic correction:
    \setbox\z@\hbox{$\macc@style{\macc@nucleus}_{}$}%
    \setbox\tw@\hbox{$\macc@style{\macc@nucleus}{}_{}$}%
    \dimen@\wd\tw@
    \advance\dimen@-\wd\z@
%Now \dimen@ is the italic correction of the symbol.
    \divide\dimen@ 3
    \@tempdima\wd\tw@
    \advance\@tempdima-\scriptspace
%Now \@tempdima is the width of the symbol.
    \divide\@tempdima 10
    \advance\dimen@-\@tempdima
%Now \dimen@ = (italic correction / 3) - (Breite / 10)
    \ifdim\dimen@>\z@ \dimen@0pt\fi
%The bar will be shortened in the case \dimen@<0 !
    \rel@kern{0.6}\kern-\dimen@
    \if#31
      \overline{\rel@kern{-0.6}\kern\dimen@\macc@nucleus\rel@kern{0.4}\kern\dimen@}%
      \advance\dimen@0.4\dimexpr\macc@kerna
%Place the combined final kern (-\dimen@) if it is >0 or if a superscript follows:
      \let\final@kern#2%
      \ifdim\dimen@<\z@ \let\final@kern1\fi
      \if\final@kern1 \kern-\dimen@\fi
    \else
      \overline{\rel@kern{-0.6}\kern\dimen@#1}%
    \fi
  }%
  \macc@depth\@ne
  \let\math@bgroup\@empty \let\math@egroup\macc@set@skewchar
  \mathsurround\z@ \frozen@everymath{\mathgroup\macc@group\relax}%
  \macc@set@skewchar\relax
  \let\mathaccentV\macc@nested@a
%The following initialises \macc@kerna and calls \mathaccent:
  \if#31
    \macc@nested@a\relax111{#1}%
  \else
%If the argument consists of more than one symbol, and if the first token is
%a letter, use that letter for the computations:
    \def\gobble@till@marker##1\endmarker{}%
    \futurelet\first@char\gobble@till@marker#1\endmarker
    \ifcat\noexpand\first@char A\else
      \def\first@char{}%
    \fi
    \macc@nested@a\relax111{\first@char}%
  \fi
  \endgroup
}
\makeatother

%% Shortened math font commands:
%% Blackboard bold math capitals
\newcommand{\bbA}{\mathbb{A}}
\newcommand{\bbB}{\mathbb{B}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbD}{\mathbb{D}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\bbF}{\mathbb{F}}
\newcommand{\bbG}{\mathbb{G}}
\newcommand{\bbH}{\mathbb{H}}
\newcommand{\bbI}{\mathbb{I}}
\newcommand{\bbJ}{\mathbb{J}}
\newcommand{\bbK}{\mathbb{K}}
\newcommand{\bbL}{\mathbb{L}}
\newcommand{\bbM}{\mathbb{M}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbO}{\mathbb{O}}
\newcommand{\bbP}{\mathbb{P}}
\newcommand{\bbQ}{\mathbb{Q}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbS}{\mathbb{S}}
\newcommand{\bbT}{\mathbb{T}}
\newcommand{\bbU}{\mathbb{U}}
\newcommand{\bbV}{\mathbb{V}}
\newcommand{\bbW}{\mathbb{W}}
\newcommand{\bbX}{\mathbb{X}}
\newcommand{\bbY}{\mathbb{Y}}
\newcommand{\bbZ}{\mathbb{Z}}

%% Bold math letters
\renewcommand{\a}{\mathbf{a}}
\renewcommand{\b}{\mathbf{b}}
\renewcommand{\c}{\mathbf{c}}
\renewcommand{\d}{\mathbf{d}}
\newcommand{\e}{\mathbf{e}}
\newcommand{\be}{\mathbf{e}}
\newcommand{\f}{\mathbf{f}}
\newcommand{\g}{\mathbf{g}}
\newcommand{\h}{\mathbf{h}}
\renewcommand{\i}{\mathbf{i}}
\renewcommand{\j}{\mathbf{j}}
\renewcommand{\k}{\mathbf{k}}
\renewcommand{\l}{\mathbf{l}}
\newcommand{\m}{\mathbf{m}}
\newcommand{\n}{\mathbf{n}}
%\renewcommand{\o}{\mathbf{o}}
\newcommand{\p}{\mathbf{p}}
\newcommand{\q}{\mathbf{q}}
\renewcommand{\r}{\mathbf{r}}
\newcommand{\s}{\mathbf{s}}
\renewcommand{\t}{\mathbf{t}}
\renewcommand{\u}{\mathbf{u}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\w}{\mathbf{w}}
\newcommand{\x}{\mathbf{x}}
\newcommand{\y}{\mathbf{y}}
\newcommand{\z}{\mathbf{z}}

\newcommand{\A}{\mathbf{A}}
\newcommand{\B}{\mathbf{B}}
\newcommand{\C}{\mathbf{C}}
\newcommand{\D}{\mathbf{D}}
\newcommand{\E}{\mathbf{E}}
\newcommand{\F}{\mathbf{F}}
\newcommand{\G}{\mathbf{G}}
\renewcommand{\H}{\mathbf{H}}
\newcommand{\I}{\mathbf{I}}
\newcommand{\J}{\mathbf{J}}
\newcommand{\K}{\mathbf{K}}
\renewcommand{\L}{\mathbf{L}}
\newcommand{\M}{\mathbf{M}}
\newcommand{\N}{\mathbf{N}}
\renewcommand{\O}{\mathbf{O}}
\renewcommand{\P}{\mathbf{P}}
\newcommand{\Q}{\mathbf{Q}}
\newcommand{\R}{\mathbf{R}}
%\renewcommand{\S}{\mathbf{S}}
\newcommand{\T}{\mathbf{T}}
\newcommand{\U}{\mathbf{U}}
\newcommand{\V}{\mathbf{V}}
\newcommand{\W}{\mathbf{W}}
\newcommand{\X}{\mathbf{X}}
\newcommand{\Y}{\mathbf{Y}}
\newcommand{\Z}{\mathbf{Z}}

%% Caligraphic math capitals
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

%% Script math capitals
\newcommand{\sA}{\mathscr{A}}
\newcommand{\sB}{\mathscr{B}}
\newcommand{\sC}{\mathscr{C}}
\newcommand{\sD}{\mathscr{D}}
\newcommand{\sE}{\mathscr{E}}
\newcommand{\sF}{\mathscr{F}}
\newcommand{\sG}{\mathscr{G}}
\newcommand{\sH}{\mathscr{H}}
\newcommand{\sI}{\mathscr{I}}
\newcommand{\sJ}{\mathscr{J}}
\newcommand{\sK}{\mathscr{K}}
\newcommand{\sL}{\mathscr{L}}
\newcommand{\sM}{\mathscr{M}}
\newcommand{\sN}{\mathscr{N}}
\newcommand{\sO}{\mathscr{O}}
\newcommand{\sP}{\mathscr{P}}
\newcommand{\sQ}{\mathscr{Q}}
\newcommand{\sR}{\mathscr{R}}
\newcommand{\sS}{\mathscr{S}}
\newcommand{\sT}{\mathscr{T}}
\newcommand{\sU}{\mathscr{U}}
\newcommand{\sV}{\mathscr{V}}
\newcommand{\sW}{\mathscr{W}}
\newcommand{\sX}{\mathscr{X}}
\newcommand{\sY}{\mathscr{Y}}
\newcommand{\sZ}{\mathscr{Z}}

%% Mathfrak letters
\newcommand{\fra}{\mathfrak{a}}
\newcommand{\frb}{\mathfrak{b}}
\newcommand{\frc}{\mathfrak{c}}
\newcommand{\frd}{\mathfrak{d}}
\newcommand{\fre}{\mathfrak{e}}
\newcommand{\frf}{\mathfrak{f}}
\newcommand{\frg}{\mathfrak{g}}
\newcommand{\frh}{\mathfrak{h}}
\newcommand{\fri}{\mathfrak{i}}
\newcommand{\frj}{\mathfrak{j}}
\newcommand{\frk}{\mathfrak{k}}
\newcommand{\frl}{\mathfrak{l}}
\newcommand{\frm}{\mathfrak{m}}
\newcommand{\frn}{\mathfrak{n}}
\newcommand{\fro}{\mathfrak{o}}
\newcommand{\frp}{\mathfrak{p}}
\newcommand{\frq}{\mathfrak{q}}
\newcommand{\frr}{\mathfrak{r}}
\newcommand{\frs}{\mathfrak{s}}
\newcommand{\frt}{\mathfrak{t}}
\newcommand{\fru}{\mathfrak{u}}
\newcommand{\frv}{\mathfrak{v}}
\newcommand{\frw}{\mathfrak{w}}
\newcommand{\frx}{\mathfrak{x}}
\newcommand{\fry}{\mathfrak{y}}
\newcommand{\frz}{\mathfrak{z}}

\newcommand{\fA}{\mathfrak{A}}
\newcommand{\frA}{\mathfrak{A}}
\newcommand{\fB}{\mathfrak{B}}
\newcommand{\frB}{\mathfrak{B}}
\newcommand{\fC}{\mathfrak{C}}
\newcommand{\fD}{\mathfrak{D}}
\newcommand{\fE}{\mathfrak{E}}
\newcommand{\fF}{\mathfrak{F}}
\newcommand{\fG}{\mathfrak{G}}
\newcommand{\fH}{\mathfrak{H}}
\newcommand{\fI}{\mathfrak{I}}
\newcommand{\fJ}{\mathfrak{J}}
\newcommand{\fK}{\mathfrak{K}}
\newcommand{\fL}{\mathfrak{L}}
\newcommand{\fM}{\mathfrak{M}}
\newcommand{\fN}{\mathfrak{N}}
\newcommand{\fO}{\mathfrak{O}}
\newcommand{\fP}{\mathfrak{P}}
\newcommand{\fQ}{\mathfrak{Q}}
\newcommand{\fR}{\mathfrak{R}}
\newcommand{\fS}{\mathfrak{S}}
\newcommand{\fT}{\mathfrak{T}}
\newcommand{\fU}{\mathfrak{U}}
\newcommand{\fV}{\mathfrak{V}}
\newcommand{\fW}{\mathfrak{W}}
\newcommand{\fX}{\mathfrak{X}}
\newcommand{\fY}{\mathfrak{Y}}
\newcommand{\fZ}{\mathfrak{Z}}


%Sans Serif Letters
\newcommand{\sfA}{\mathsf{A}}
\newcommand{\sfB}{\mathsf{B}}
\newcommand{\sfC}{\mathsf{C}}
\newcommand{\sfD}{\mathsf{D}}
\newcommand{\sfE}{\mathsf{E}}
\newcommand{\sfF}{\mathsf{F}}
\newcommand{\sfG}{\mathsf{G}}
\newcommand{\sfH}{\mathsf{H}}


%Script Lower Case
\newcommand{\scrj}{\mathscr{j}}
\newcommand{\scrk}{\mathscr{k}}
\newcommand{\scrl}{\mathscr{l}}
\newcommand{\scrv}{\mathscr{v}}
\newcommand{\scrs}{\mathscr{s}}

%% Additional Commands
\newcommand{\hc}{\textnormal{h.c.}}
\newcommand{\defeq}{\vcentcolon=}
\DeclareMathOperator{\re}{Re}
\DeclareMathOperator{\res}{Res}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\co}{co}
\DeclareMathOperator{\cch}{\overline{co}}
\renewcommand{\slash}{\slashed}
\newcommand{\tn}[1]{\textnormal{#1}}
\newcommand{\textdef}[1]{\textit{\textbf{#1}}}
\newcommand{\unit}[1]{\,\textnormal{#1}}
\newcommand{\qedalt}{\renewcommand{\qedsymbol}{$\blacksquare$}}
\newcommand{\qedblank}{\renewcommand{\qedsymbol}{$\square$}}
\DeclareMathOperator{\image}{im}
\DeclareMathOperator{\im}{im}
\DeclareMathOperator{\codim}{codim}
\DeclareMathOperator{\ind}{ind}
\DeclareMathOperator{\nul}{nul}
\DeclareMathOperator{\defect}{def}
\DeclareMathOperator{\asc}{ascent}
\DeclareMathOperator{\dsc}{descent}
\renewcommand{\mathring}[1]{\accentset{\circ}{#1}}
\DeclareMathOperator{\vecspan}{span}
\renewcommand{\qedsymbol}{$\blacksquare$}
\newcommand{\id}{\mathrm{id}}
\newcommand{\Unitary}{\mathrm{U}}
\newcommand{\Un}{\Unitary}
\DeclareMathOperator{\PU}{\mathbb{P}\mathrm{U}}
\newcommand{\class}[1]{\llbracket #1 \rrbracket}

\DeclareMathOperator{\Log}{Log}
\DeclareMathOperator*{\colim}{colim}
\DeclareMathOperator{\diam}{diam}
\DeclareMathOperator{\GL}{\mathrm{GL}}

\newcommand{\1}{\mathds{1}}
\newcommand{\sa}{\mathrm{sa}}
\newcommand{\Int}{\mathfrak{Int}}
\DeclareMathOperator{\Aut}{\mathrm{Aut}}
\DeclareMathOperator{\Inn}{Inn}

%ray product
\newcommand{\ltrans}{|\!\langle}
\newcommand{\rtrans}{\rangle\!|}
\newcommand{\ray}[1]{\ltrans #1 \rtrans}
\newcommand{\chd}{\mathrm{chd}}
\newcommand{\FS}{\mathrm{FS}}
\newcommand{\gap}{\mathrm{gap}}

\begin{comment}
\DeclareMathAlphabet{\mathboondoxcal}{U}{BOONDOX-cal}{m}{n}
\SetMathAlphabet{\mathboondoxcal}{bold}{U}{BOONDOX-cal}{b}{n}
\DeclareMathAlphabet{\mathbboondoxcal} {U}{BOONDOX-cal}{b}{n}
\newcommand{\scrj}{\mathboondoxcal{j}}
\newcommand{\scrk}{\mathboondoxcal{k}}
\newcommand{\scrl}{\mathboondoxcal{l}}
\newcommand{\scrv}{\mathboondoxcal{v}}
\newcommand{\scrs}{\mathboondoxcal{s}}
\end{comment}


\DeclareMathAlphabet{\mathrsfs}{U}{rsfs}{m}{n}
\DeclareMathAlphabet{\mathrsfso}{U}{rsfso}{m}{n}

\newcommand{\pset}{\wp}
\newcommand{\npset}{\mathcal{P}_+}
\newcommand{\fpset}{\mathcal{P}_0}
\newcommand{\nfpset}{\mathcal{P}_0}

\newcommand{\hilbG}{\mathscr{G}}
\newcommand{\hilbH}{\mathscr{H}}
\newcommand{\hilbK}{\mathscr{K}}
\newcommand{\state}{\mathrsfs{S}}
\newcommand{\pstate}{\mathrsfs{P}}
\newcommand{\folium}{\mathrsfs{F}}
\newcommand{\sector}{\mathrsfs{Q}}

\newcommand{\ball}{\mathbb{B}}
\newcommand{\disk}{\mathbb{D}}
\newcommand{\sphere}{\mathbb{S}}

\newcommand{\interval}{I}
\newcommand{\denmat}[1]{DM_{#1}(\bbC)}
\newcommand{\htpy}[1]{\simeq_{#1}}
\newcommand{\pathhtpy}[1]{\simeq_{p,#1}}
\DeclareMathOperator{\diag}{\mathrm{diag}}
\DeclareMathOperator{\Ad}{\mathrm{Ad}}

\newcommand{\UHFQ}{\bbQ}
\newcommand{\projective}{\bbS}

\newcommand{\proj}{\tn{proj}}
\newcommand{\Set}{\mathsf{Set}}
\newcommand{\refine}{r}
\newcommand{\parbra}[1]{\prescript{}{\hilbK}{\bra{#1}}}
\newcommand{\parket}[1]{\ket{#1}_{\hilbK}}


